Conditional Computation for Continual Learning

Catastrophic forgetting of connectionist neural networks is caused by the global sharing of parameters among all training examples. In this study, we analyze parameter sharing under the conditional computation framework where the parameters of a neural network are conditioned on each input example. At one extreme, if each input example uses a disjoint set of parameters, there is no sharing of parameters thus no catastrophic forgetting. At the other extreme, if the parameters are the same for every example, it reduces to the conventional neural network. We then introduce a clipped version of maxout networks which lies in the middle, i.e. parameters are shared partially among examples. Based on the parameter sharing analysis, we can locate a limited set of examples that are interfered when learning a new example. We propose to perform rehearsal on this set to prevent forgetting, which is termed as conditional rehearsal. Finally, we demonstrate the effectiveness of the proposed method in an online non-stationary setup, where updates are made after each new example and the distribution of the received example shifts over time.

==> sections/intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-10pt}
\vspace{\sectionReduceTop}
\section{Introduction}
\label{sec:intro}
\vspace{\sectionReduceBot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Continual learning is the ability to learn from a stream of data with continuously shifting distributions. Catastrophic forgetting has been a key obstacle to continual learning in connectionist neural networks.
While there is no established theory regarding the cause of catastrophic forgetting in neural networks, the global sharing of parameters among all training samples leads to the changes of the previously obtained representations, which, in our opinion, might contribute to the forgetting issue.

% One popular approach for alleviating catastrophic forgetting relies on rehearsal on historical examples \cite{Shin2017}.
% Regularization has also been proposed in several previous works \cite{Kirkpatrick2017,Li2017}, which protects weights by adding constraints to the loss function.

One key observation that motivates our investigation here is that we can reduce forgetting if we sparsify the updates to the weights by means of node sharpening \cite{French1991}, dropout \cite{Goodfellow2013}, maxout \cite{Goodfellow2013} or competing to compute \cite{Srivastava2013}.
Although empirically, it does exhibit certain capability of mitigating the forgetting, the results are still far from being satisfactory \cite{Goodfellow2013}.
We argue that sparsely updating neurons does not change the fact that the parameters associated with these neurons are still shared by all historical examples.


%%%%%%%%%%%%%

As suggested in \cite{Parisi2018}, existing methods to mitigate forgetting can be classified into three categories: a) Retraining with regularization; b) Training with expansion; c) Selective network retraining and expansion. 
Our proposed method, however, does not belong to any one of the three categories, as it selectively retrains networks \textit{without} expansion. 

The contributions of this work are:
\begin{itemize}
  \item We develop conditional computation as a general framework for analyzing catastrophic forgetting.
  \item Based on the conditional computation interpretation, we propose conditional rehearsal which is more efficient than random rehearsal.
  \item We propose to use rehearsal over hypernetwork for multi-task training.
  \item Last but not least, we analyze ``maxout network'' within this framework, and proposed a method that learns without forgetting on streaming examples.
\end{itemize}

==> sections/sup.tex <==
\section{Implementation Details}

\cite{Jayram2018} introduces a \textit{bookmarks} to store previous attention vectors. 
